The fabulous world of GKP codes

Quantum error correction is an essential ingredient in the development of quantum technologies. Its subject is to investigate ways to embed quantum Hilbert spaces into a physical system such that this subspace is robust against small imperfections in the physical systems. This task is exceedingly complex: for one, this is due to the vast diversity of possible physical systems with different structure to use. For another, every physical setting also comes with its own imperfections that need to be protected against. Bred by the complexity of a technological ambition, research on quantum error correction has developed into a large field of research that ranges from engineering of small systems with a single photon to the creation of macroscopic topological phases of matter and models of complex emergent physics. A quintessential tool in quantum error correction is the stabilizer formalism, which tames quantum systems by enforcing symmetries. A Gottesman-Kitaev-Preskill (GKP) code is a stabilizer code that creates a logical subspace within an infinite dimensional Hilbert space by endowing it with translational symmetries. While in practice the infinitude of the Hilbert space, as well as the infinitude of the translational symmetry group are considered as obstacles for implementation, in theory these are precisely the features that make the theory of GKP codes particularly rich, well behaved and well-connected to fascinating topics in mathematics. The purpose of this thesis is to explore these connections: to understand the coding theoretic and practical properties of GKP codes, utilizing its rich mathematical foundation, and to provide a foundation for future research. Along this journey we discover -- through the looking glass of GKP codes -- how quantum error correction fits into a fabulous mathematical world and formulate a series of dreams about possible directions of research.

==> HallEffect.tex <==
\subsection{GKP Hamiltonians and the Hall effect}

Throughout this chapter I have often mentioned a link between the GKP code and physics underlying the quantum Hall effect. Since this a highly interesting connection and potentially relevant for future research, is is appropriate to explain the key steps in deriving this connection. The following derivation presents a simplified version of a discussion in ref.~\cite{Ganeshan2016}. 

Consider the approximate GKP Hamiltonian 
\begin{equation}
H=\epsilon \frac{\bs{\hat{x}}^{\dagger}\bs{\hat{x}}}{2} - U\sum_{k=1}^{2n} \cos \lr{\sqrt{2\pi} \bs{\xi}_k^T J \bs{\hat{x}}}.
\end{equation}
We use the trick that every basis for a GKP code can be written as $M=\lr{D\oplus I_n} S_1^T$ with a symplectic matrix $S_1$, and apply a Gaussian unitary with symplectic transformation $S=S_1^TS_0$ where $S_0=\lr{\sqrt{2\pi}^{-1}I_n\oplus \sqrt{2\pi}I_n}$ and $D=\diag\lr{d_1,\hdots, d_n}$, we can compute

\begin{equation}
U^{\dagger}_{S} H U_{S} = \epsilon \frac{\bs{\hat{x}}^{\dagger}S^TS \bs{\hat{x}}}{2} -U\sum_{k=1}^{n} \cos\lr{d_k\hat{p}_k}+\cos\lr{2\pi \hat{q}_k}\label{eq:H_traf}
\end{equation}




The periodic part of this Hamiltonian naturally commutes with displacement operators in $\Z^n \oplus D^{-1}\Z^n$, and it becomes convenient to define a generalization of the co-called Zak-basis \cite{Zak1967} with $\bs{\theta}, \bs{\phi} \in \left[0, 2\pi\right)^n$

\begin{equation}
\ket{\bs{\theta}, \bs{\phi}}= \frac{1}{\lr{2\pi}^{n/2}}\sum_{\bs{j}\in \Z^{n}} e^{i\bs{j}^T\bs{\theta}} \ket{\bs{j}+\bs{\phi}/2\pi}_{\bs{q}},
\end{equation}
where the ket $\ket{\bs{x}}_{\bs{q}}=\bigotimes_{i=1}^n \ket{q_i}_q$ denotes the $n$-dimensional position eigenstate.

These states are eigenstates of the commuting operators $e^{i\hat{p}_k}, e^{i2\pi \hat{q}_l},\; \forall k,l = 1\hdots n$ with
\begin{align}
e^{i\hat{p}_k}\ket{\bs{\theta}, \bs{\phi}}&= e^{i\theta_k} \ket{\bs{\theta}, \bs{\phi}},\\
e^{i2\pi\hat{q}_l}\ket{\bs{\theta}, \bs{\phi}}&= e^{i\phi_l} \ket{\bs{\theta}, \bs{\phi}},
\end{align}
and simple displacements act as
\begin{align}
e^{i\bs{a}^T\bs{\hat{q}}} \ket{\bs{\theta}, \bs{\phi}} =e^{i\bs{a}^T\bs{\phi}/2\pi} \ket{\bs{\theta}+\bs{a}, \bs{\phi}}\\
e^{i\bs{b}^T\bs{\hat{p}}} \ket{\bs{\theta}, \bs{\phi}} = \ket{\bs{\theta}, \bs{\phi}-2\pi \bs{b}}.\label{eq:disp_zak}
\end{align}

The states $\ket{\bs{\theta}, \bs{\phi}}$ form a complete basis, as can be checked by computing

\begin{align}
\int_{\left[0, 2\pi\right)^{2n}} d\bs{\theta}d\bs{\phi}\, \ket{\bs{\theta}, \bs{\varphi}}\bra{\bs{\theta}, \bs{\varphi}} 
&=\sum_{\bs{j},\bs{j'}\in \Z^{n}}  \int_{\left[0, 2\pi\right)^n}d\bs{\varphi}\, \lrq{\frac{1}{\lr{2\pi}^{n}}\int_{\left[0, 2\pi\right)^n} d\bs{\theta}e^{i\lr{\bs{j}-\bs{j'}}^T\bs{\theta}} }
\nonumber \\ &\hspace{2cm} \ket{\bs{j}+\bs{\varphi}/2\pi}_{\bs{q}}\bra{\bs{j'}+\bs{\varphi}/2\pi}_{\bs{q}} \nonumber \\
&= \sum_{\bs{j}\in \Z^{n}}\int_{\left[0, 2\pi\right)^n} \ket{\bs{j}+\bs{\varphi}/2\pi}_{\bs{q}}\bra{\bs{j}+\bs{\varphi}/2\pi}_{\bs{q}} \nonumber \\
&= \hat{I},
\end{align}
where the expression in the square brackets evaluates to $\delta_{\bs{j}, \bs{j'}}$, and in this basis the quadrature variables become represented by
\begin{equation}
\bs{\hat{x}}=\begin{pmatrix}
-\bs{\hat{p}_{\theta}} + \bs{\hat{\varphi}}/2\pi \\ 2\pi \bs{\hat{p}_{\varphi}}
\end{pmatrix}=\bs{\hat{p}_{\theta, \phi}} + \bs{A}\lr{\bs{\hat{\varphi}}},
\end{equation}
where the momenta of the compact variables are represented by $\hat{p}_{\theta_k}\equiv -i\partial_{\theta_k}$ and $\hat{p}_{\varphi_k}\equiv -i\partial_{\varphi_k}$ such that (when exponentiated) they behave as if $\lrq{\hat{\theta}_k, \hat{p}_{\theta_l}}=\lrq{\hat{\varphi}_k, \hat{p}_{\varphi_l}}=i\delta_{kl}$.
In the Zak representation, it holds that 
\begin{equation}
e^{i2\pi \hat{p}_{\theta_k}}=\hat{I}, \hspace{1cm}  e^{i2\pi \hat{p}_{\varphi_k}}=e^{i\hat{\theta}_k} ,
\end{equation}
as can be checked using eq.~\eqref{eq:disp_zak}, such that also
\begin{equation}
e^{i2\pi \hat{q}_k}=e^{i\hat{\phi}_k},\hspace{1cm} e^{id_k\hat{p}_k}=e^{id_k\hat{\theta}_k}.
\end{equation}

Combining all of these points, the Hamiltonian in eq.~\eqref{eq:H_traf} becomes
\begin{equation}
H'=\frac{\epsilon}{2} \lr{\bs{\hat{p}_{\theta, \phi}} + \bs{A}\lr{\bs{\hat{\varphi}}}}^{\dagger}S^TS\lr{\bs{\hat{p}_{\theta, \varphi}} + \bs{A}\lr{\bs{\hat{\varphi}}}} -U\sum_{k=1}^{n}  \cos\lr{d_k\hat{\theta}_k}+\cos\lr{ \hat{\varphi}_k},
\end{equation}
which describes the motion of $n$ particles with generalized total quadrature $\bs{\hat{\Theta}}=\bs{\hat{\theta}}\oplus\bs{\hat{\varphi}}$ in the cosine potential on the $n$-torus $[0,2\pi)^{2n}$. In the simple case of diagonal $C=S^TS$, we recognize that $\bs{A}\lr{\bs{\hat{\varphi}}}$ takes the role of a vector potential which can be interpreted to describes the presence of a magnetic field driving these particles, while for non-diagonal these  `mechanical momenta' $\bs{\hat{\pi}}=\bs{\hat{p}_{\theta, \phi}} + \bs{A}\lr{\bs{\hat{\varphi}}}$ couple non-trivially. 

==> SCPhotonBasics.tex <==
\chapter*{Interlude: Photonics and Superconducting Circuit Basics}
\addcontentsline{toc}{chapter}{Interlude: Photonics and Superconducting Circuit Basics}  

